Context-based Transformer Models for Answer Sentence Selection

An important task for the design of Question Answering systems is the selection of the sentence containing (or constituting) the answer from documents relevant to the asked question. Most previous work has only used the target sentence to compute its score with the question as the models were not powerful enough to also effectively encode additional contextual information. In this paper, we analyze the role of the contextual information in the sentence selection task, proposing a Transformer based architecture that leverages two types of contexts, local and global. The former describes the paragraph containing the sentence, aiming at solving implicit references, whereas the latter describes the entire document containing the candidate sentence, providing content-based information. The results on three different benchmarks show that the combination of local and global contexts in a Transformer model significantly improves the accuracy in Answer Sentence Selection.

==> charts_squad.tex <==


\begin{figure}[!ht]
\centering
%\resizebox{\textwidth}{!}{


\begin{tikzpicture}
        \begin{customlegend}
        	[legend columns=2,legend style={align=center,column sep=2ex},
        	legend entries={Transformer, \textsc{Loc\_T}, \textsc{Glob\_b}, \textsc{Glob\_e}, Dual-CTX}]
        \addlegendimage{red, line width=1pt}
        \addlegendimage{blue, line width=1pt}
        \addlegendimage{orange, line width=1pt,dashed}
        \addlegendimage{green, line width=1pt,dashed}
        \addlegendimage{cyan, line width=1pt}
        \end{customlegend}
\end{tikzpicture}

\begin{tikzpicture}
	\begin{axis}[
	        name=plotLeft,
			scale=0.65,
			xlabel=epoch,
			ylabel=MAP,
			%ytick={0.66, 0.68, 0.70,0.72},
			grid=both,
			xtick={1,5,10,15,20},
			ymin=0.93,
			xmax=20,
			ylabel near ticks,
			tick label style={font=\scriptsize},
			xlabel style={yshift=1ex},
			title={\normalsize SQuAD},
			title style={yshift=-1.5ex,},
		]
		
		\addplot [cyan]
		    table[x=epo, y=map,] {results/squad_mixbow.txt};
		%\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/squad_mixbow.txt};
		%\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/squad_mixbow.txt};
		%\addplot [fill=cyan!20] fill between[of=upper_wbt and lower_wbt];
		
		\addplot [green,dashed]
		    table[x=epo, y=map,] {results/squad_globalaver.txt};
		%\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_globalaver.txt};
		%\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_globalaver.txt};
		%\addplot [fill=green!20] fill between[of=upper_wbt and lower_wbt];
		
		\addplot [orange,dashed]
		    table[x=epo, y=map,] {results/squad_globalbow.txt};
		%\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_globalbow.txt};
		%\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_globalbow.txt};
		%\addplot [fill=orange!20] fill between[of=upper_wbt and lower_wbt];

		\addplot [red]
		    table[x=epo, y=map,] {results/squad_baseline.txt};
		\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/squad_baseline.txt};
		\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/squad_baseline.txt};
		\addplot [fill=red!20] fill between[of=upper_wbt and lower_wbt];
		
		\addplot [blue]
		    table[x=epo, y=map] {results/squad_tuples.txt};
		%\addplot [name path=upper_wtt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_tuples.txt};
		%\addplot [name path=lower_wtt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_tuples.txt};
		%\addplot [fill=blue!20] fill between[of=upper_wtt and lower_wtt];
		

		
		

	\end{axis}
\end{tikzpicture}
%}
\caption{MAP results on SQuAD.}
\label{fig:res_squad}
\end{figure}

==> charts_wikiqa.tex <==


\begin{figure}[!ht]
\centering
%\resizebox{\textwidth}{!}{


\begin{tikzpicture}
        \begin{customlegend}
        	[legend columns=2,legend style={align=center,column sep=2ex},
        	legend entries={Transformer, \textsc{Loc\_T}, \textsc{Glob\_b}, \textsc{Glob\_e}, Dual-CTX}]
        \addlegendimage{red, line width=1pt}
        \addlegendimage{blue, line width=1pt}
        \addlegendimage{orange, line width=1pt,dashed}
        \addlegendimage{green, line width=1pt,dashed}
        \addlegendimage{cyan, line width=1pt}
        \end{customlegend}
\end{tikzpicture}

\begin{tikzpicture}
	\begin{axis}[
	        name=plotLeft,
			scale=0.65,
			xlabel=epoch,
			ylabel=MAP,
			%ytick={0.66, 0.68, 0.70,0.72},
			grid=both,
			xtick={1,10, 20,30,40},
			ymin=0.64,
			xmax=50,
			ylabel near ticks,
			tick label style={font=\scriptsize},
			xlabel style={yshift=1ex},
			title={\normalsize WikiQA},
			title style={yshift=-1.5ex,},
		]
		
		\addplot [cyan]
		    table[x=epo, y=map,] {results/wikiqa_mixbow.txt};
		\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_mixbow.txt};
		\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_mixbow.txt};
		\addplot [fill=cyan!20] fill between[of=upper_wbt and lower_wbt];
		
		\addplot [green,dashed]
		    table[x=epo, y=map,] {results/wikiqa_globalaver.txt};
		%\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_globalaver.txt};
		%\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_globalaver.txt};
		%\addplot [fill=green!20] fill between[of=upper_wbt and lower_wbt];
		
		\addplot [orange,dashed]
		    table[x=epo, y=map,] {results/wikiqa_globalbow.txt};
		%\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_globalbow.txt};
		%\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_globalbow.txt};
		%\addplot [fill=orange!20] fill between[of=upper_wbt and lower_wbt];

		\addplot [red]
		    table[x=epo, y=map,] {results/wikiqa_baseline.txt};
		\addplot [name path=upper_wbt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_baseline.txt};
		\addplot [name path=lower_wbt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_baseline.txt};
		\addplot [fill=red!20] fill between[of=upper_wbt and lower_wbt];
		
		\addplot [blue]
		    table[x=epo, y=map] {results/wikiqa_tuples.txt};
		%\addplot [name path=upper_wtt,draw=none] table[x=epo,y expr=\thisrow{map}+\thisrow{map_std}] {results/wikiqa_tuples.txt};
		%\addplot [name path=lower_wtt,draw=none] table[x=epo,y expr=\thisrow{map}-\thisrow{map_std}] {results/wikiqa_tuples.txt};
		%\addplot [fill=blue!20] fill between[of=upper_wtt and lower_wtt];
		

		
		

	\end{axis}
\end{tikzpicture}
%}
\caption{MAP results on WikiQA (without TANDA) for local, global contexts, and the complete architecture. Due to graphical issues, the standard deviation is shown only for the Transformer and the final model.}
\label{fig:res_wikiqa}
\end{figure}
